Gaia EDR3 in 6D: Searching for unbound stars in the Galaxy

The early third data release (EDR3) of the European Space Agency satellite Gaia provides coordinates, parallaxes, and proper motions for ~1.47 billion sources in our Milky Way, based on 34 months of observations. The combination of Gaia DR2 radial velocities with the more precise and accurate astrometry provided by Gaia EDR3 makes the best dataset available to search for the fastest nearby stars in our Galaxy. We compute the velocity distribution of ~7 million stars with precise parallaxes, to investigate the high-velocity tail of the velocity distribution of stars in the Milky Way. We release a catalogue with distances, total velocities, and corresponding uncertainties for all the stars considered in our analysis, available at https://sites.google.com/view/tmarchetti/research . By applying quality cuts on the Gaia astrometry and radial velocities, we identify a clean subset of 94 stars with a probability Pub > 50% to be unbound from our Galaxy. 17 of these have Pub > 80% and are our best candidates. We propagate these stars in the Galactic potential to characterize their orbits. We find that 11 stars are consistent with being ejected from the Galactic disk, and are possible hyper-runaway star candidates. The other 6 stars are not consistent with coming from a known star-forming region. We investigate the effect of adopting a parallax zero point correction, which strongly impacts our results: when applying this correction, we identify only 12 stars with Pub > 50%, 3 of these having Pub > 80%. Spectroscopic follow-ups with ground-based telescopes are needed to confirm the candidates identified in this work.

==> Fastest stars in Gaia EDR3/tab_candidates_0.8.tex <==
\begin{landscape}
\begin{table}
\centering
\caption{Observed and derived properties for the clean sample of 17 high velocity stars with a probability $P_\mathrm{ub} > 0.8$ of being unbound from the Milky Way. Quantities derived from the orbital integration are reported in Table \ref{tab:candidates_orb}. Stars are ordered by decreasing values of $P_\mathrm{ub}$.}
\label{tab:candidates}

\begin{threeparttable}
\setlength{\tabcolsep}{4pt}

\begin{tabular}{lcccccccccccc}

\hline
{\Gaia} EDR3 ID & (RA, Dec.) & ($l$, $b$) & $\varpi$ & $\mu_{\alpha*}$ & $\mu_\delta$ & $v_\mathrm{rad}$ & $G$ & $d$ & $r_\mathrm{GC}$ & $v_\mathrm{GC}$ & $P_\mathrm{MW}$ & $P_\mathrm{ub}$ \\
 & ($^\circ$) & ($^\circ$) & (mas) & (mas yr$^{-1}$) & (mas yr$^{-1}$) & (km s$^{-1}$) & (mag) & (pc) & (pc) & (\kms) &  &  \\
\hline

\textbf{Galactic} \\[0.15cm]

1383279090527227264 & ($240.337$, $41.167$) & ($65.46$, $48.85$) & $0.131 \pm 0.013$ & $-25.726 \pm 0.013$ & $-9.655 \pm 0.016$ & $-180.902 \pm 2.421$ & $13.0$ & $7644^{+834}_{-712}$ & $9511^{+499}_{-387}$ & $810^{+109}_{-93}$ & $1.0$ & $1.0$ \\[0.15cm] 

1375165725506487424 & ($231.849$, $36.034$) & ($57.9$, $55.86$) & $0.101 \pm 0.013$ & $-15.14 \pm 0.011$ & $-14.147 \pm 0.015$ & $-84.773 \pm 0.435$ & $11.19$ & $9895^{+1466}_{-1093}$ & $10767^{+1065}_{-728}$ & $761^{+144}_{-107}$ & $0.92$ & $0.99$ \\[0.15cm] 

1591615309672292224 & ($222.64$, $49.359$) & ($85.17$, $58.12$) & $0.103 \pm 0.014$ & $-15.377 \pm 0.013$ & $-13.192 \pm 0.018$ & $-123.121 \pm 0.403$ & $11.08$ & $9706^{+1485}_{-1156}$ & $12376^{+1156}_{-848}$ & $727^{+142}_{-111}$ & $0.97$ & $0.98$ \\[0.15cm] 

6703116567945367808 & ($273.431$, $-50.811$) & ($343.16$, $-15.15$) & $0.104 \pm 0.014$ & $-7.239 \pm 0.013$ & $-22.238 \pm 0.012$ & $209.079 \pm 2.936$ & $13.38$ & $9669^{+1474}_{-1169}$ & $3789^{+998}_{-524}$ & $849^{+161}_{-127}$ & $1.0$ & $0.97$ \\[0.15cm]

4337459232822884992 & ($249.981$, $-10.467$) & ($6.8$, $23.1$) & $0.118 \pm 0.015$ & $-19.142 \pm 0.017$ & $-14.857 \pm 0.013$ & $-290.985 \pm 0.411$ & $12.5$ & $8454^{+1226}_{-924}$ & $3469^{+537}_{-148}$ & $779^{+134}_{-99}$ & $1.0$ & $0.96$ \\[0.15cm] 

5847216962695435392 & ($207.66$, $-68.85$) & ($308.26$, $-6.59$) & $0.094 \pm 0.014$ & $-15.919 \pm 0.012$ & $-7.314 \pm 0.016$ & $260.077 \pm 18.159$ & $14.11$ & $10650^{+1822}_{-1365}$ & $8543^{+1301}_{-835}$ & $734^{+151}_{-113}$ & $1.0$ & $0.94$ \\[0.15cm] 

6065230602133664000 & ($203.583$, $-55.6$) & ($309.01$, $6.77$) & $0.125 \pm 0.012$ & $-21.301 \pm 0.012$ & $-6.024 \pm 0.013$ & $103.959 \pm 1.088$ & $13.22$ & $7977^{+862}_{-718}$ & $6972^{+400}_{-267}$ & $675^{+90}_{-75}$ & $0.65$ & $0.92$ \\[0.15cm] 

6090995247640198016 & ($212.05$, $-49.143$) & ($315.62$, $11.83$) & $0.117 \pm 0.018$ & $-16.81 \pm 0.02$ & $8.515 \pm 0.02$ & $21.091 \pm 0.523$ & $12.4$ & $8502^{+1509}_{-1125}$ & $6452^{+788}_{-406}$ & $689^{+129}_{-95}$ & $1.0$ & $0.87$ \\[0.15cm] 

2123569205674089856 & ($275.497$, $49.44$) & ($77.63$, $24.87$) & $0.074 \pm 0.011$ & $-9.826 \pm 0.012$ & $3.583 \pm 0.015$ & $-87.772 \pm 0.543$ & $11.66$ & $13505^{+2227}_{-1717}$ & $14343^{+1899}_{-1393}$ & $597^{+107}_{-82}$ & $1.0$ & $0.86$ \\[0.15cm] 

6193551030782723072 & ($201.24$, $-23.677$) & ($312.76$, $38.55$) & $0.09 \pm 0.015$ & $-13.149 \pm 0.017$ & $-0.749 \pm 0.01$ & $412.704 \pm 2.601$ & $13.12$ & $11172^{+2247}_{-1573}$ & $9718^{+1698}_{-1039}$ & $619^{+125}_{-83}$ & $1.0$ & $0.82$ \\[0.15cm] 

1477675943342041472 & ($213.484$, $31.892$) & ($52.76$, $71.46$) & $0.111 \pm 0.014$ & $-17.034 \pm 0.015$ & $-8.538 \pm 0.014$ & $71.542 \pm 5.089$ & $12.9$ & $9019^{+1300}_{-1037}$ & $10914^{+926}_{-680}$ & $613^{+114}_{-89}$ & $1.0$ & $0.82$ \\[0.15cm]



\textbf{Extragalactic} \\[0.15cm]

1297316350890352000 & ($248.178$, $21.272$) & ($38.97$, $39.59$) & $0.083 \pm 0.013$ & $-6.321 \pm 0.011$ & $-14.085 \pm 0.013$ & $-335.072 \pm 1.086$ & $12.96$ & $12053^{+2091}_{-1556}$ & $9693^{+1638}_{-1090}$ & $721^{+147}_{-107}$ & $0.0$ & $0.96$ \\[0.15cm]

3644492029415356032 & ($211.82$, $-4.143$) & ($336.18$, $53.76$) & $0.101 \pm 0.017$ & $7.943 \pm 0.018$ & $-12.983 \pm 0.014$ & $76.86 \pm 1.14$ & $11.36$ & $9896^{+2046}_{-1530}$ & $8773^{+1409}_{-869}$ & $687^{+141}_{-102}$ & $0.0$ & $0.93$ \\[0.15cm] 

4450458649852400640 & ($242.697$, $7.16$) & ($19.52$, $38.78$) & $0.139 \pm 0.014$ & $3.357 \pm 0.013$ & $-23.11 \pm 0.011$ & $-119.88 \pm 1.25$ & $12.94$ & $7206^{+751}_{-657}$ & $5647^{+211}_{-107}$ & $674^{+80}_{-69}$ & $0.0$ & $0.92$ \\[0.15cm] 

3859294747025975552 & ($161.032$, $6.306$) & ($241.66$, $53.29$) & $0.176 \pm 0.021$ & $4.94 \pm 0.025$ & $-27.251 \pm 0.025$ & $-98.225 \pm 5.147$ & $10.8$ & $5690^{+763}_{-628}$ & $11161^{+558}_{-441}$ & $620^{+93}_{-74}$ & $0.0$ & $0.90$ \\[0.15cm] 

2038763839481341056 & ($290.711$, $29.843$) & ($62.97$, $6.98$) & $0.064 \pm 0.011$ & $-4.285 \pm 0.01$ & $-8.479 \pm 0.012$ & $-9.172 \pm 3.509$ & $13.3$ & $15663^{+3231}_{-2285}$ & $14019^{+2849}_{-1898}$ & $641^{+138}_{-96}$ & $0.0$ & $0.90$ \\[0.15cm] 

6571360298580575104 & ($331.235$, $-42.701$) & ($357.05$, $-52.95$) & $0.139 \pm 0.016$ & $-13.125 \pm 0.013$ & $-18.851 \pm 0.014$ & $-1.458 \pm 1.936$ & $11.98$ & $7188^{+937}_{-746}$ & $6883^{+367}_{-212}$ & $639^{+98}_{-78}$ & $0.0$ & $0.83$ \\[0.15cm] 




\hline
\end{tabular}

\begin{tablenotes}

\item \emph{Note.} Distances and total velocities are quoted in terms of the median of the distribution, with uncertainties derived from the $16$th and $84$th percentiles.

\end{tablenotes}

\end{threeparttable}
\end{table}
\end{landscape}

==> Fastest stars in Gaia EDR3/tab_candidates_0.8_orb.tex <==
\begin{table*}
	
	\caption{Galactocentric cylindrical coordinates $(R_\mathrm{GC}, z_\mathrm{GC})$,  energy per unit mass $E$, minimum crossing radius $r_\mathrm{min}$, ejection velocity $v_\mathrm{ej}$, and flight time $t_\mathrm{F}$ for the clean sample of 17 stars with $P_\mathrm{ub} > 0.8$. Stars are ordered as in Table \ref{tab:candidates}.}
	
	\label{tab:candidates_orb}
	
	\begin{threeparttable}
	\setlength{\tabcolsep}{12pt}
		
		\begin{tabular}{lcccccc}
		
		\hline
        {\Gaia} EDR3 ID & $R_\mathrm{GC}$ & $z_\mathrm{GC}$ & $E$ & $r_\mathrm{min}$ & $v_\mathrm{ej}$ & $t_\mathrm{F}$ \\
         & (pc) & (pc) & (kpc$^2$ Myr$^{-2}$) & (pc) & (km s$^{-1}$) & (Myr) \\
\hline

\textbf{Galactic} \\[0.15cm]

1383279090527227264 & $7558^{+138}_{-88}$ & $5774^{+627}_{-535}$ & $0.191^{+0.106}_{-0.074}$ & $12412^{+1163}_{-908}$ & $796^{+113}_{-89}$ & $10.9^{+0.3}_{-0.2}$\\[0.15cm] 

1375165725506487424 & $6972^{+191}_{-81}$ & $8205^{+1212}_{-904}$ & $0.16^{+0.131}_{-0.079}$ & $20020^{+3117}_{-2204}$ & $728^{+148}_{-104}$ & $21.0^{+0.2}_{-0.2}$\\[0.15cm]

1591615309672292224 & $9211^{+400}_{-276}$ & $8265^{+1261}_{-981}$ & $0.143^{+0.128}_{-0.086}$ & $19106^{+2819}_{-2214}$ & $708^{+148}_{-118}$ & $19.7^{+0.5}_{-0.4}$\\[0.15cm] 

6703116567945367808 & $2821^{+973}_{-412}$ & $-2529^{+309}_{-389}$ & $0.172^{+0.167}_{-0.106}$ & $6188^{+3522}_{-2005}$ & $819^{+152}_{-104}$ & $10.4^{+1.8}_{-1.2}$\\[0.15cm] 

4337459232822884992 & $1198^{+504}_{-210}$ & $3317^{+478}_{-360}$ & $0.122^{+0.125}_{-0.078}$ & $12498^{+2840}_{-2086}$ & $708^{+141}_{-99}$ & $16.0^{+0.2}_{-0.2}$\\[0.15cm] 

5847216962695435392 & $8456^{+1284}_{-821}$ & $-1218^{+159}_{-213}$ & $0.122^{+0.148}_{-0.087}$ & $5582^{+1571}_{-868}$ & $766^{+150}_{-104}$ & $5.9^{+0.2}_{-0.2}$\\[0.15cm] 

6065230602133664000 & $6907^{+390}_{-258}$ & $949^{+100}_{-83}$ & $0.066^{+0.067}_{-0.052}$ & $17538^{+22501}_{-7955}$ & $596^{+33}_{-30}$ & $35.4^{+30.32}_{-10.4}$\\[0.15cm] 

6090995247640198016 & $6211^{+732}_{-359}$ & $1749^{+306}_{-228}$ & $0.076^{+0.102}_{-0.065}$ & $5593^{+776}_{-381}$ & $706^{+118}_{-88}$ & $3.1^{+0.0}_{-0.0}$\\[0.15cm] 

2123569205674089856 & $13163^{+1663}_{-1207}$ & $5697^{+935}_{-721}$ & $0.055^{+0.076}_{-0.05}$ & $13305^{+2065}_{-1497}$ & $606^{+100}_{-74}$ & $9.6^{+0.0}_{-0.1}$\\[0.15cm] 

6193551030782723072 & $6771^{+994}_{-493}$ & $6970^{+1397}_{-978}$ & $0.046^{+0.098}_{-0.054}$ & $3468^{+4863}_{-2429}$ & $702^{+63}_{-9}$ & $17.4^{+3.6}_{-2.2}$\\[0.15cm] 
 
1477675943342041472 & $6758^{+109}_{-116}$ & $8570^{+1232}_{-983}$ & $0.057^{+0.089}_{-0.055}$ & $12836^{+3625}_{-2507}$ & $612^{+109}_{-73}$ & $23.3^{+1.2}_{-1.0}$\\[0.15cm] 




\textbf{Extragalactic} \\[0.15cm]

1297316350890352000 & $5907^{+959}_{-506}$ & $7685^{+1329}_{-989}$ & $0.124^{+0.132}_{-0.087}$ & - & - & - \\[0.15cm]

3644492029415356032 & $3648^{+465}_{-322}$ & $7990^{+1647}_{-1231}$ & $0.099^{+0.118}_{-0.07}$ & - & - & - \\[0.15cm] 

4450458649852400640 & $3382^{+330}_{-316}$ & $4522^{+469}_{-410}$ & $0.058^{+0.071}_{-0.046}$ & - & - & - \\[0.15cm] 

3859294747025975552 & $10173^{+328}_{-263}$ & $4591^{+612}_{-504}$ & $0.059^{+0.071}_{-0.047}$ & - & - & - \\[0.15cm] 

2038763839481341056 & $13889^{+2822}_{-1878}$ & $1906^{+388}_{-274}$ & $0.09^{+0.106}_{-0.077}$ & - & - & - \\[0.15cm] 

6571360298580575104 & $3821^{+445}_{-558}$ & $-5725^{+597}_{-750}$ & $0.049^{+0.079}_{-0.051}$ & - & - & - \\[0.15cm] 


\hline
		
		\end{tabular}
		
		\begin{tablenotes}

\item \emph{Note.} Derived quantities are quoted in terms of the median of the distribution, with uncertainties derived from the $16$th and $84$th percentiles.

\end{tablenotes}
		
	\end{threeparttable}
	
\end{table*}

==> Fastest stars in Gaia EDR3/tab_candidates_0.8_zp.tex <==
\begin{landscape}
\begin{table}
%\centering
\caption{Observed and derived properties for the clean sample of 12 high velocity stars with a probability $P_\mathrm{ub} > 0.5$ of being unbound from the Milky Way, computed including the estimate of the parallax zero point $\varpi_\mathrm{zp}$. Stars are ordered by decreasing values of $P_\mathrm{ub}$.}
\label{tab:candidates_zp}

\begin{threeparttable}
\setlength{\tabcolsep}{5pt}

\begin{tabular}{lccccccccccccc}

\hline
{\Gaia} EDR3 ID & (RA, Dec.) & ($l$, $b$) & $\varpi - \varpi_\mathrm{zp}$ & $\mu_{\alpha*}$ & $\mu_\delta$ & $v_\mathrm{rad}$ & $G$ & $d$ & $r_\mathrm{GC}$ & $v_\mathrm{GC}$ & $P_\mathrm{MW}$ & $P_\mathrm{ub}$ \\
 & ($^\circ$) & (mas) & (mas yr$^{-1}$) & (mas yr$^{-1}$) & (km s$^{-1}$) & (mag) & (pc) & (pc) & (\kms) &  &  \\
\hline

\textbf{Galactic} \\[0.15cm]

6014438731195297408 & ($233.205$, $-33.907$) & ($337.33$, $17.97$) & $0.118 \pm 0.017$ & $-15.224 \pm 0.018$ & $-7.848 \pm 0.014$ & $-253.194 \pm 8.513$ & $12.94$ & $10693^{+2307}_{-1609}$ & $5278^{+1766}_{-922}$ & $729^{+170}_{-112}$ & $1.0$ & $0.88$ \\[0.15cm] 

4337459232822884992 & ($249.981$, $-10.467$) & ($6.8$, $23.1$) & $0.14 \pm 0.015$ & $-19.142 \pm 0.017$ & $-14.857 \pm 0.013$ & $-290.985 \pm 0.411$ & $12.5$ & $7745^{+992}_{-752}$ & $3359^{+213}_{-48}$ & $702^{+107}_{-79}$ & $1.0$ & $0.86$ \\[0.15cm]

1383279090527227264 & ($240.337$, $41.167$) & ($65.46$, $48.85$) & $0.199 \pm 0.013$ & $-25.726 \pm 0.013$ & $-9.655 \pm 0.016$ & $-180.902 \pm 2.421$ & $13.0$ & $6071^{+521}_{-451}$ & $8710^{+243}_{-190}$ & $606^{+68}_{-59}$ & $1.0$ & $0.84$ \\[0.15cm] 

6090995247640198016 & ($212.05$, $-49.143$) & ($315.62$, $11.83$) & $0.139 \pm 0.018$ & $-16.81 \pm 0.02$ & $8.515 \pm 0.02$ & $21.091 \pm 0.523$ & $12.4$ & $7807^{+1239}_{-935}$ & $6180^{+528}_{-256}$ & $630^{+105}_{-78}$ & $1.0$ & $0.71$ \\[0.15cm] 

6901673112193397248 & ($309.967$, $-10.203$) & ($35.99$, $-28.68$) & $0.118 \pm 0.017$ & $6.933 \pm 0.018$ & $-10.591 \pm 0.013$ & $-455.382 \pm 2.084$ & $12.88$ & $10726^{+2468}_{-1711}$ & $7572^{+1805}_{-993}$ & $587^{+125}_{-79}$ & $1.0$ & $0.62$ \\[0.15cm] 

1375165725506487424 & ($231.849$, $36.034$) & ($57.9$, $55.86$) & $0.156 \pm 0.013$ & $-15.14 \pm 0.011$ & $-14.147 \pm 0.015$ & $-84.773 \pm 0.435$ & $11.19$ & $7789^{+832}_{-710}$ & $9429^{+497}_{-385}$ & $555^{+81}_{-69}$ & $1.0$ & $0.59$ \\[0.15cm] 

6257153998879080320 & ($226.415$, $-18.787$) & ($341.93$, $33.73$) & $0.101 \pm 0.015$ & $-9.219 \pm 0.018$ & $-9.861 \pm 0.015$ & $336.968 \pm 1.76$ & $12.15$ & $11315^{+2420}_{-1620}$ & $6977^{+1867}_{-1023}$ & $560^{+138}_{-86}$ & $0.96$ & $0.50$ \\[0.15cm]

\textbf{Extragalactic} \\[0.15cm]

6241679678390298880 & ($236.994$, $-20.512$) & ($349.46$, $26.01$) & $0.103 \pm 0.014$ & $-9.69 \pm 0.017$ & $-11.065 \pm 0.012$ & $-304.986 \pm 0.815$ & $12.59$ & $11410^{+2293}_{-1552}$ & $5691^{+1862}_{-1037}$ & $642^{+141}_{-89}$ & $0.22$ & $0.73$ \\[0.15cm] 

1204061267883975040 & ($238.111$, $20.197$) & ($33.45$, $48.2$) & $0.129 \pm 0.014$ & $-9.756 \pm 0.013$ & $-14.42 \pm 0.015$ & $-262.04 \pm 0.835$ & $12.92$ & $9713^{+1547}_{-1172}$ & $8518^{+1023}_{-660}$ & $604^{+124}_{-92}$ & $0.44$ & $0.72$ \\[0.15cm]

4182243409716233856 & ($296.209$, $-15.205$) & ($24.94$, $-18.54$) & $0.102 \pm 0.013$ & $-9.511 \pm 0.016$ & $-11.653 \pm 0.012$ & $-135.681 \pm 1.457$ & $12.63$ & $11279^{+1854}_{-1429}$ & $5972^{+1446}_{-929}$ & $613^{+131}_{-101}$ & $0.41$ & $0.61$ \\[0.15cm] 

1309092223502856576 & ($257.42$, $29.977$) & ($52.3$, $33.99$) & $0.084 \pm 0.01$ & $-5.097 \pm 0.011$ & $-6.631 \pm 0.012$ & $-485.643 \pm 0.523$ & $12.73$ & $14885^{+2634}_{-1991}$ & $12843^{+2277}_{-1616}$ & $524^{+87}_{-60}$ & $0.24$ & $0.56$ \\[0.15cm]

4200563090205883392 & ($290.3$, $-9.399$) & ($27.84$, $-10.85$) & $0.093 \pm 0.014$ & $-10.489 \pm 0.016$ & $-8.89 \pm 0.014$ & $-194.05 \pm 1.165$ & $12.31$ & $11553^{+2208}_{-1586}$ & $6038^{+1785}_{-1068}$ & $585^{+141}_{-100}$ & $0.33$ & $0.52$ \\[0.15cm] 



 



 
\hline
\end{tabular}

\begin{tablenotes}

\item \emph{Note.} Distances and total velocities are quoted in terms of the median of the distribution, with uncertainties derived from the $16$th and $84$th percentiles.

\end{tablenotes}

\end{threeparttable}
\end{table}
\end{landscape}

==> Fastest stars in Gaia EDR3/tab_catalogue.tex <==
\begin{table*}
	
	\caption{Description of the columns of the catalogue with distances and velocities. Entries labelled $^1$ are taken directly from the {\Gaia} EDR3 catalogue, while entries labelled $^2$ are derived in this paper. We refer the interested reader to Section \ref{sec:method} for details on how these quantities are computed. For the entries labelled $^2$, the quoted values correspond to the median of the distribution, with lower and upper uncertainties computed, respectively, from the $16$th and the $84$th percentile. Column 60 is present only in the version of the catalogue which includes the effect of the parallax zero point.}
	
	\label{tab:catalogue}
	
	\begin{threeparttable}
	\setlength{\tabcolsep}{12pt}
		
		\begin{tabular}{llll}
		
			\hline		
			Column & Units & Name & Description \\
			\hline
			
			% Gaia DR2:
			
			1 & - & source\_id & {\Gaia} EDR3 identifier$^1$ \\
			2 & deg & ra & Right ascension$^1$ \\
			3 & deg & dec & Declination$^1$ \\
			4 & mas & parallax & Parallax$^1$ \\
			5 & mas & e\_parallax & Standard uncertainty in parallax$^1$ \\
			6 & mas yr$^{-1}$ & pmra & Proper motion in right ascension$^1$ \\
			7 & mas yr$^{-1}$ & e\_pmra & Standard uncertainty in proper motion in right ascension$^1$ \\
			8 & mas yr$^{-1}$ & pmdec & Proper motion in declination$^1$ \\
			9 & mas yr$^{-1}$ & e\_pmdec & Standard uncertainty in proper motion in declination$^1$ \\
			10 & - & corr\_parallax\_pmra & Correlation between parallax and proper motion in right ascension$^1$\\
			11 & - & corr\_parallax\_pmdec & Correlation between parallax and proper motion in declination$^1$\\
			12 & - & corr\_pmra\_pmdec & Correlation between proper motion in right ascension and proper motion in declination$^1$\\
			13 & km s$^{-1}$ & vrad & {\Gaia} DR2 Radial velocity$^1$ \\
			14 & km s$^{-1}$ & e\_vrad & {\Gaia} DR2 Radial velocity error$^1$ \\
			15 & mag & GMag & G-band mean magnitude$^1$ \\
			16 & mag & BPMag & BP-band mean magnitude$^1$ \\
			17 & mag & RPMag & RP-band mean magnitude$^1$ \\
			18 & - & \textsc{ruwe} & Renormalised Unit Weight Error$^1$ \\
			19 & - & \textsc{rv\_nb\_transits} & Number of epochs used in {\Gaia} DR2 to determine the radial velocity$^1$ \\
			
			% Distances:
			
			20 & pc & dist & Distance estimate$^2$ \\
			21 & pc & el\_dist & Lower uncertainty on distance$^2$ \\
			22 & pc & eu\_dist & Upper uncertainty on distance$^2$ \\
			23 & pc & rGC & Spherical Galactocentric radius$^2$ \\
			24 & pc & el\_rGC & Lower uncertainty on spherical Galactocentric radius$^2$ \\
			25 & pc & eu\_rGC & Upper uncertainty on spherical Galactocentric radius$^2$ \\
			26 & pc & RGC & Cylindrical Galactocentric radius$^2$ \\
			27 & pc & el\_RGC & Lower uncertainty on cylindrical Galactocentric radius$^2$ \\
			28 & pc & eu\_RGC & Upper uncertainty on cylindrical Galactocentric radius$^2$ \\
			29 & pc & xGC & Cartesian Galactocentric $x$-coordinate$^2$ \\
			30 & pc & el\_xGC & Lower uncertainty on Cartesian Galactocentric $x$-coordinate$^2$ \\
			31 & pc & eu\_xGC & Upper uncertainty on Cartesian Galactocentric $x$-coordinate$^2$ \\		
			32 & pc & yGC & Cartesian Galactocentric $y$-coordinate$^2$ \\
			33 & pc & el\_yGC & Lower uncertainty on Cartesian Galactocentric $y$-coordinate$^2$ \\
			34 & pc & eu\_yGC & Upper uncertainty on Cartesian Galactocentric $y$-coordinate$^2$ \\
			35 & pc & zGC & Cartesian Galactocentric $z$-coordinate$^2$ \\
			36 & pc & el\_zGC & Lower uncertainty on Cartesian Galactocentric $z$-coordinate$^2$ \\
			37 & pc & eu\_zGC & Upper uncertainty on Cartesian Galactocentric $z$-coordinate$^2$ \\
		
			% Velocities:
			
			38 & km s$^{-1}$ & U & Cartesian Galactocentric $x$-velocity$^2$ \\
			39 & km s$^{-1}$ & el\_U & Lower uncertainty on Cartesian Galactocentric $x$-velocity$^2$ \\
			40 & km s$^{-1}$ & eu\_U & Upper uncertainty on Cartesian Galactocentric $x$-velocity$^2$ \\
			41 & km s$^{-1}$ & V & Cartesian Galactocentric $y$-velocity$^2$ \\
			42 & km s$^{-1}$ & el\_V & Lower uncertainty on Cartesian Galactocentric $y$-velocity$^2$ \\
			43 & km s$^{-1}$ & eu\_V & Upper uncertainty on Cartesian Galactocentric $y$-velocity$^2$ \\
			44 & km s$^{-1}$ & W & Cartesian Galactocentric $z$-velocity$^2$ \\
			45 & km s$^{-1}$ & el\_W & Lower uncertainty on Cartesian Galactocentric $z$-velocity$^2$ \\
			46 & km s$^{-1}$ & eu\_W & Upper uncertainty on Cartesian Galactocentric $z$-velocity$^2$ \\
			47 & km s$^{-1}$ & UW & Cartesian Galactocentric $xz$-velocity$^2$ \\
			48 & km s$^{-1}$ & el\_UW & Lower uncertainty on Cartesian Galactocentric $xz$-velocity$^2$ \\
			49 & km s$^{-1}$ & eu\_UW & Upper uncertainty on Cartesian Galactocentric $xz$-velocity$^2$ \\ 	
			50 & km s$^{-1}$ & vR & Cylindrical Galactocentric $R$-velocity$^2$ \\
			51 & km s$^{-1}$ & el\_vR & Lower uncertainty on cylindrical Galactocentric $R$-velocity$^2$ \\
			52 & km s$^{-1}$ & eu\_vR & Upper uncertainty on cylindrical Galactocentric $R$-velocity$^2$ \\
			53 & km s$^{-1}$ & vphi & Cylindrical Galactocentric azimuthal velocity$^2$ \\
			54 & km s$^{-1}$ & el\_vphi & Lower uncertainty on cylindrical Galactocentric azimuthal velocity$^2$ \\
			55 & km s$^{-1}$ & eu\_vphi & Upper uncertainty on cylindrical Galactocentric azimuthal velocity$^2$ \\			
			
			56 & km s$^{-1}$ & vtot & Total velocity in the Galactic rest-frame$^2$ \\
			57 & km s$^{-1}$ & el\_vtot & Lower uncertainty on total velocity in the Galactic rest-frame$^2$ \\
			58 & km s$^{-1}$ & eu\_vtot & Upper uncertainty on total velocity in the Galactic rest-frame$^2$ \\
			
			59 & - & P\_ub & Probability of being unbound from the Galaxy$^2$ \\
			
			60 & mas & parallax\_zp & Parallax zero point, estimated as in \citet{Lindegren+20b} \\

			\hline
		
		\end{tabular}
		
	\end{threeparttable}
	
\end{table*}
